Characterizing the Properties and Constitution of Compact Objects in Gravitational-Wave Binaries

Astrophysical observations point toward strong evidence for the existence of black holes (BHs). Nevertheless, it is yet to be established or ruled out with confidence whether some exotic compact objects (ECOs), capable of mimicking black holes from an observational point of view, are indeed doing so. In classical General Relativity (GR), a horizon is the defining feature of a black hole, which prevents any event inside from causally affecting the outside Universe. The quest for distinguishing black holes from horizonless compact objects using gravitational wave (GW) signals from compact binary coalescences (CBCs) can be helped by utilizing the phenomenon of tidal heating (TH), which leaves its imprint on the binary waveforms through the horizon parameters. First, we study the measurabilities of these parameters within the inspiral regime. Then, to extend our investigation for heavier binaries, we construct an inspiral-merger-ringdown waveform by using post-Newtonian calculations for the inspiral and numerical relativity data for the merger-ringdown part that incorporates the effects of tidal heating of black holes in the phase and the amplitude. The new model shows improvements in waveform accuracy when compared to numerical relativity data. In the late inspiral phase when the compact objects are closer to each other, the effects of tidal heating are stronger, opening up the possibility of identifying the objects more precisely. We demonstrate, from numerical relativity data of binary black holes, how one can model tidal heating in the late inspiral regime and leverage this knowledge to test for horizonless compact objects mimicking black holes. These studies bear significance in determining the nature of compact objects having masses in the entire range that LIGO and future ground-based gravitational-wave detectors can detect.

==> 00_Cover/frontcover.tex <==
% This is the cover page which will be printed
% on the cover of a soft or hard or leather binding
\newcommand{\ttitle}{Characterizing the Properties and Constitution
of Compact Objects in Gravitational-Wave Binaries}
\newcommand{\authorname}{Samanwaya Mukherjee}
\newcommand{\cosupname}{Prof. Sukanta Bose}
\newcommand{\supname}{Prof. Gulab Chand Dewangan}
\newcommand{\degreename}{Doctor of Philosophy}

\begin{center}
\includegraphics[scale=0.3]{IUCAA-logo.png}\\
{\fontencoding{T1}\fontfamily{pzc}\fontseries{m}\fontshape{n}\selectfont
\Huge \bfseries Doctoral Thesis}\\
\vspace*{1cm}
{\hrule width \hsize height 2pt \kern 1mm \hrule width \hsize height 1pt}

\vspace*{0.25cm}
{\huge \bfseries \scshape \ttitle}
\vspace*{\fill}
\begin{flushright}
{\LARGE \bfseries \itshape Samanwaya Mukherjee}
\end{flushright}
\vspace*{0.25cm}

{\hrule width \hsize height 1pt \kern 1mm \hrule width \hsize height 2pt}

\end{center}

%% Page 2 : Blank
\newpage\null\newpage
% \cleardoublepage


==> 02_Approval/Approval.tex <==
% Page 5 : Approval of the DAC

% \chapter*{} is needed to link the hyperlinks in contents to the corresponding pages properly.
\chapter*{}
\vspace{-1cm} % Increase if the dept. letterhead requires more space
% \thispagestyle{empty}

{\centering \includegraphics[width=\linewidth, scale=1]{iitbbs_letterhead}}
{\hrule width \hsize height 1.5pt \kern .5mm \hrule width \hsize height 1.5pt}

\vspace{2ex}
\begin{center}
    \textbf{\Large APPROVAL OF THE VIVA VOCE BOARD}
\end{center}

\begin{flushright}
    Date: \thisdate\today/\thismonthdigit\today/\thisyear\today
    % % To leave blank space for inserting the date later,
    % % comment the line above and uncomment the line below 
    % Date: \space\space\space/\space\space\space\space/\thisyear\today
\end{flushright}

\par Certified that the thesis entitled ``\textbf{Write Thesis Title Here}", submitted by \textbf{John Doe} to the \textbf{Indian Institute of Technology Bhubaneswar}, for the award of the degree of \textit{Doctor of Philosophy} has been accepted by the external examiners and that the student has successfully defended the thesis in the viva voce examination held today.

% DAC Members
\vspace*{1em}
\begin{center}
    \begin{minipage}[t]{0.31\textwidth}
    \begin{flushleft}
        \hrule\vspace{2ex}
        {\small {\bfseries Dr. DAC Member 1}\\
        (Member, DAC)\\
        Designation\\
        School of Awesome Sciences\\
        IIT Bhubaneswar}
    \end{flushleft}
    \end{minipage}
    \hfill
    \begin{minipage}[t]{0.31\textwidth}
    \begin{center}
        \hrule\vspace{2ex}
        {\small {\bfseries Dr. DAC Member 2}\\
        (Member, DAC)\\
        Designation\\
        School of Awesome Sciences\\
        IIT Bhubaneswar}
    \end{center}
    \end{minipage}
    \hfill
    \begin{minipage}[t]{0.31\textwidth}
    \begin{flushright}
        \hrule\vspace{2ex}
        {\small {\bfseries Dr. DAC Member 3}\\
        (Member, DAC)\\
        Designation\\
        2nd School of Awesome Sciences\\
        IIT Bhubaneswar}
    \end{flushright}
    \end{minipage}
\end{center}

% Supervisor(s)
\vspace*{15pt}
\begin{center}
    % Comment out the following mini-page if you
    % have two supervisors
    \begin{minipage}[t]{0.4\textwidth}
    \begin{center}
        \hrule\vspace{2ex}
        {\small {\bfseries Dr. Supervisor 1}\\
        (Supervisor)\\
        Designation\\
        School of Awesome Sciences\\
        IIT Bhubaneswar}
    \end{center}
    \end{minipage}

    % % Uncomment the following two mini-pages if you
    % % have two supervisors
    % \begin{minipage}[t]{0.4\textwidth}
    %     \hrule\vspace{2ex}
    %     \begin{flushleft}
    %     {\small {\bfseries Dr. Supervisor 1}\\
    %     (Supervisor)\\
    %     Designation\\
    %     School of Awesome Sciences\\
    %     IIT Bhubaneswar}
    %     \end{flushleft}
    % \end{minipage}
    % \hfill
    % \begin{minipage}[t]{0.4\textwidth}
    %     \begin{flushright}
    %     \hrule\vspace{2ex}
    %     {\small {\bfseries Dr. Supervisor 2}\\
    %     (Co-supervisor)\\
    %     Designation\\
    %     2nd School of Awesome Sciences\\
    %     IIT Bhubaneswar}
    %     \end{flushright}
    % \end{minipage}
\end{center}

% Chair and External Examiners
\vspace*{15pt}
\begin{center}
\begin{minipage}[t]{0.4\textwidth}
    \hrule\vspace{2ex}
    \begin{flushleft}
    {\small {\bfseries Dr. External Examiner}\\
    (External Examiner)\\
    Designation\\
    Awesome Department\\
    Awesome Institute}
    \end{flushleft}
\end{minipage}
\hfill
\begin{minipage}[t]{0.4\textwidth}
    \begin{flushright}
    \hrule\vspace{2ex}
    {\small {\bfseries Dr. Head of Department}\\
    (Chairman, DAC)\\
    Designation\\
    School of Awesome Sciences\\
    IIT Bhubaneswar}
    \end{flushright}
\end{minipage}
\end{center}

\addcontentsline{toc}{chapter}{Approval Of The Viva voce Board}

%% Page 6 : Blank
\newpage
\thispagestyle{empty}
\null\newpage
% \cleardoublepage


==> 08_Symbols/Symbols.tex <==
%% Symbols
\nomenclature{$\nabla$}{Vector differential operator}
\nomenclature{$\vec{u}$}{velocity of fluid}
\nomenclature{$\vec{u}_{ev}$}{Electro-viscous velocity}

\nomenclature{$\vec{F}_{ST}$}{Forces due to Surface tension at the interface}
\nomenclature{$\vec{F}_{ST}$}{Forces due to electrical stresses}
\nomenclature{$\rho$}{Density of fluid}
\nomenclature{$p$}{Fluid pressure}
\nomenclature{$\mu$}{Dynamic viscosity}
\nomenclature{$\nu$}{Kinematic viscosity}

\nomenclature{$\Gamma$}{Interface between liquid and vapour}
\nomenclature{$\gamma$}{Coefficient of surface tension}
\nomenclature{$k$}{Curvature of the interface}
\nomenclature{$\hat{n}$}{unit vector pointing normal direction to an interface}
\nomenclature{$\hat{t}$}{unit vector pointing tangential direction to an interface}

\nomenclature{$\rho_i$}{Density of dispersed phase}
\nomenclature{$\rho_o$}{Density of continuous phase}
\nomenclature{$Re$}{Reynolds number}
\nomenclature{$Ca_e$}{Electric capillary number}
\nomenclature{$Re$}{Reynolds number}
\nomenclature{$Re$}{Reynolds number}
\nomenclature{$\tau$}{Relaxation time}


==> 110_Publications/Publications.tex <==

\defbibheading{subbibliography}{\section{#1}}
\defbibfilter{booksandchapters}{%
( type=book or type=incollection )
}
\defbibfilter{papers}{%
 ( type=article or type=unpublished )
}
\defbibfilter{conferences}{%
 ( type=inproceedings )
}

\pagestyle{fancy}
\fancyhf{}
\fancyhead[RE]{\bfseries Publications}
\fancyhead[LO]{\bfseries Publications}
\fancyhead[LE,RO]{\thepage}

\chapter*{Publications}
%% Add the BibTeX entries to the file pub.bib
%% for your own journal articles, books, chapters
%% and proceedings etc. They will be automatically
%% sorted and added to the thesis by the
%% following refsection

\begin{refsection}[110_Publications/pub.bib]
    % Since, with the chapter numbers, the table of contents
    % look ugly, the following four lines remove the chapter
    % numbers leaving only the section number
    \addtocontents{toc}{\protect\renewcommand{\protect\cftchappresnum}{}}
    \renewcommand{\chaptername}{Chapter}
    \renewcommand{\thesection}{\arabic{section}}
    \setcounter{section}{0}
    
    \addcontentsline{toc}{chapter}{Publications}
    \nocite{*}
    %% Uncomment the following line to add journal articles
    \printbibliography[heading={subbibliography},title={Journal Articles},filter={papers},resetnumbers=true]
    
    %% Uncomment the following line to add Conference Proceedings
    % \printbibliography[heading={subbibliography},title={Conference Proceedings},filter={conferences},resetnumbers=true]
    
    %% Uncomment the following line to add books and chapters
    % \printbibliography[heading={subbibliography},title={Books and Chapters},filter={booksandchapters},resetnumbers=true]
\end{refsection}

